Why is AI not a Panacea for Data Workers? An Interview Study on Human-AI Collaboration in Data Storytelling

Data storytelling plays an important role in data workers' daily jobs since it boosts team collaboration and public communication. However, to make an appealing data story, data workers spend tremendous efforts on various tasks, including outlining and styling the story. Recently, a growing research trend has been exploring how to assist data storytelling with advanced artificial intelligence (AI). However, existing studies may focus on individual tasks in the workflow of data storytelling and do not reveal a complete picture of humans' preference for collaborating with AI. To better understand real-world needs, we interviewed eighteen data workers from both industry and academia to learn where and how they would like to collaborate with AI. Surprisingly, though the participants showed excitement about collaborating with AI, many of them also expressed reluctance and pointed out nuanced reasons. Based on their responses, we first characterize stages and tasks in the practical data storytelling workflows and the desired roles of AI. Then the preferred collaboration patterns in different tasks are identified. Next, we summarize the interviewees' reasons why and why not they would like to collaborate with AI. Finally, we provide suggestions for human-AI collaborative data storytelling to hopefully shed light on future related research.

==> sources/outdated/04-finding-workflow_role-v2.tex <==
\begin{figure*}[h!]
    \centering
    \includegraphics[width=\linewidth]{figs/task-role-v6.pdf}
    \caption{
    This figure summarizes participants' opinions about where and how they would like to collaborate with AI.
    (a) demonstrates AI collaborators' roles against AI's automation levels and humans' agency levels.
    (b) shows tasks in the existing workflows of our interviewees and (c) illustrates the expected AI collaborators' roles and their tasks.
    In (a), we use fully manual story creation and Heer's ideal ``agency plus automation'' collaboration mode~\cite{heer2019agency} as two anchor points and derive the relative rough positions of other roles.
    Both y-axes in (b) and (c) are the tasks in the data storytelling workflow. In (c), the heatmap presents the breakdown frequency of task-role tuples. The bar chart on the top counts the frequency of roles, while the one on the right shows the frequency of tasks. Notably, since each participant can propose multiple roles of AI collaborators for one task, the count of tasks can be larger than the number of participants. 
    }
    \vspace{-1em}
    \label{fig:task-role}
\end{figure*}

\section{Results}
This section targets answering the research questions with interview results. 
We introduce the participants' workflow (Sec.~\ref{sec:workflow}) to ground results for our research questions, \ie, where, how (Sec.~\ref{sec:where_and_how}), and why or why not~(Secs.~\ref{sec:why} and~\ref{sec:why_not}) data workers would like to collaborate with AI for data storytelling.
Overviews of results are in Fig.~\ref{fig:task-role} and Fig.~\ref{fig:why_why_not}.
% Sec.~\ref{sec:workflow} illustrates the interviewees' common workflow of data storytelling to ground results for our research questions.
% Then we attempt to answer the first research question by summarizing the roles of AI collaborators and where AI can take the roles according to interviewees' \re{opinions}~(Sec.~\ref{sec:where_and_how}).
% Fig.~\ref{fig:task-role} shows the summary of results in Sec.~\ref{sec:workflow} and Sec.~\ref{sec:where_and_how}.
% Next, Sec.~\ref{sec:why} and Sec.~\ref{sec:why_not} present interviewees' reasons about why and why not they would like to collaborate with AI, which is outlined in 
% Fig.~\ref{fig:why_why_not}.
% In this section, we label participants' IDs for opinions they expressed (P1-P18).

\subsection{What is the general workflow of data storytelling?}\label{sec:workflow}
In the first part of the interviews, we invite the participants to share their workflow of data storytelling.
\re{Most of them frequently use slide decks as the format of their data stories.
Some other formats of data stories include reports and articles.}
\re{When authoring data stories, they used slide tools (all participants), including Microsoft Powerpoint and Google Slides, and programming tools, such as Python and D3 (ten participants).
Microsoft Excel is also a common tool used by six participants.
More details are in Table~\ref{tab:demographic}.}
\re{Based on our participants' introduction to their workflows, we summarize the general workflow as three stages and seven tasks.}
Fig.~\ref{fig:task-role}(b) presents the frequency of tasks mentioned by our interviewees.

The first stage in the workflow is \textbf{planning}, where the interviewees comprehend their results from data analysis and brainstorm the overall picture of a data story.
In this stage, the interviewees commonly first \textit{decide on the core message of the data story} based on their data findings and the broader context of their projects, such as the background and the target.
After having a clearer core idea of the story, they move on to \textit{collecting supportive data facts}. 
% \revise{Following previous research~\cite{wang2019datashot}, here we define data facts as quantitative results from data analysis.}
\revise{In this paper, we consider \textit{data facts} as those quantitative results from data analysis or data-related information collected from other materials such as news.}
% These data facts mainly come from their analysis and sometimes are collected in related materials such as news.
When the supportive information is ready, the next task is to \textit{compile the story outline}, where the interviewees organize the related information according to their topics and logical relationship.
After the three tasks, the interviewees have a plan for their data story.

In the second stage, the interviewees \textbf{execute} the plans created in the first stage.
They commonly first \textit{prepare story pieces} using the collected information in the first stage.
Unlike the task of collecting related information, this task transforms collected facts into a presentable format.
For example, they draft the introduction to their background and methods.
They also design and make charts to facilitate the delivery of their findings.
The next task is to \textit{integrate story pieces},
where the interviewees may make presentation slides or reports to accommodate the story pieces according to the outline.
In this step, some supportive information that is irrelevant to the data may be added to the data story.
For example, when making slides, it is common to add pages for the title, section, and outline pages to facilitate the audience's understanding.
To make the data story more effective and appealing, at the end of the execution stage, the interviewees often \textit{style the data story}.
Some examples of styling the story include adjusting the layout of visual elements, unifying the color usage, annotating the charts, and applying animations.
Notably, the interviewees may review the results at the end of each task and iteratively improve the results.
At the end of this stage, the interviewees have complete data stories that can be shared with other stakeholders.

In the final stage, the interviewees \textbf{communicate} their data stories with others.
After finishing and checking the story, the authors will \textit{share the story} informally or formally.
When sharing the story informally with the team, the authors often want to seek advice on improving the story quality, such as the core message's clearness and the content's completeness.
Then the authors may perform the previous tasks again to refine their story.
When the stories are shared formally, multiple actions can be taken according to the sharing format.
For example, if the sharing is a live talk or video recording, it is possibly necessary to write scripts and rehearse the presentation.
When the story is shared as a document, the authors may need to upload it to the cloud or send it to others through communication software.

Though we attempt to divide the workflow into stages and tasks according to their chronological order, the procedure of data storytelling is not always linear.
Most of the time, the interviewees may experience conducting several tasks back and forth to polish their data stories.
For example, it is quite common that in the styling task, the authors can go back to prepare story pieces according to a more unified style.
Another example is that the authors may share the story with their teams several times.
They can review the story outline before execution to improve the story iteratively in an agile manner.
For example, P2 mentioned that he often communicated with team members to review his stories in different stages, including planning and execution:
\begin{displayquote}
\textit{``The first thing is to really decide what you want to focus on, right?... 
Or which data you want to focus on showing... 
I actually use paper to take some notes or some ideas. And then I prefer to
discuss with someone else.''}


\textit{``and trying to make [findings] visual...
But then you still need to see
if they work into the framework that you want to explain.
Sometimes, maybe there is some step missing or sometimes some of the visuals are not clear enough.
So I also tried to discuss with someone and got some feedback.''
}
\end{displayquote}
Reviewing and improving data stories was also considered an opportunity to gain new ideas or identify potential problems in their data analysis by some participants.
For example, P13 mentioned:
\begin{displayquote}
    \textit{``When I am reviewing [the data story], I can have some new insights. Then I need to verify these ideas with some new experiments.''}
\end{displayquote}
With these steps, his understanding of the problem could be enhanced.


We also notice that some participants, under certain scenarios, may not conduct some tasks, as shown in Fig.~\ref{fig:task-role}(b).
They may skip some steps according to the nature of their stories, such as the target audience's backgrounds and whether the story is communicated in a formal occasion.
For example, P5 mentioned that she might not integrate story pieces into slides or reports when discussing findings with her supervisor.
She instead showed several charts and presented the messages directly.
The reason was that they discussed a familiar project in an informal meeting.

\revise{Our summarized workflow mostly aligns with the previous research~\cite{lee2015more, chevalier2018analysis}, where they propose the entire lifecycle from data exploration to data storytelling.
They outlined three stages in their lifecycle, exploring data, authoring a story, and presenting a story and introduced tasks in each stage.
We refer our readers to their papers for more details.
To better fit the focus of our research, our workflow has several changes over theirs.
First, since we focus on human-AI collaboration in data storytelling, we did not explicitly interview our participants about their workflow of data exploration.
Therefore, we use the task of collecting data facts to conclude all tasks in data exploration.
Second, we add an additional \re{task} of styling the data story.
The reason is that the task was often mentioned as the one where AI can perform as collaborators.
For example, eight participants (P2, P3, P7, P8, P14-P17) mentioned that they welcomed AI's help in optimizing styles of data stories~(see Sec.~\ref{sec:ai_tasks} for more details).
Therefore, we consider that styling the data story is worth more emphasis under our scope and add it as an individual task.}
% We divide the step of ``building presentation'' in Chaveliar~\etal~\cite{chevalier2018analysis} into integrating story pieces and styling the data story.}

% \revise{Compared to previous workflow~\cite{lee2015more, chevalier2018analysis}, we have xxx differences}
% \haotian{I am a little stuck in this point. @Yun, can you fill in a little or shall we just remove this part?}

% \haotian{I updated this part.}





\subsection{Where and how do humans want to collaborate with AI?}\label{sec:where_and_how}
% % To answer our first research question, we summarize the proposed roles of AI collaborators by interviewees to illustrate how data workers would like to collaborate with AI~(Sec.~\ref{sec:ai_roles}).
Through our interview, we realized that the desired collaboration approaches depend on different tasks where humans would like to collaborate with AI.
As a result, we report the results of the first two research questions together in this section.
We first summarize the proposed roles of AI collaborators by interviewees to illustrate how data workers would like to collaborate with AI~(Sec.~\ref{sec:ai_roles}).
Then we take one step further to examine our interviewees' preferences towards the collaboration approach in different tasks of their workflow~(Sec.~\ref{sec:ai_tasks}).
% As a result, in this section, we first introduces the 


% we introduce our interviewees' preferences towards the collaboration approach in different tasks of their workflow in Sec.~\ref{sec:ai_tasks}.



\subsubsection{What are AI collaborators' roles?}\label{sec:ai_roles}


According to our interviews, the desired roles of AI can be categorized into four types, \textit{creator}, \textit{optimizer}, \textit{assistant}, and \textit{reviewer}.
The characterization of roles reflects how humans would like to \re{distribute} the work in data storytelling between AI collaborators and themselves.
\revise{In this section, we mainly provide a conceptual description of these roles.
Examples of these roles in different tasks of data storytelling from our interviews are available in Table~\ref{tab:roles_tasks}.}

The first role of AI is the \textbf{creator}. 
When AI collaborators are assigned to a task in the workflow of data storytelling, they finish the entire task independently.
The responsibility of humans is limited to providing the raw materials as input and reviewing the AI-created output.
In other words, humans are not involved in the creation process.

The second role of AI collaborators is the \textbf{optimizer}. 
When AI collaborators act as optimizers, they do not handle the entire task but take the duty of fine-tuning humans' created content.
AI optimizers need to understand the input content and then improve the content.
In this collaboration mode, humans bear more workload and outsource optimization to AI.

The third role of AI collaborators is the \textbf{reviewer}.
Under this role, AI evaluates the task performance of humans and suggests potential issues or improvements.
Compared to AI optimizers, reviewers do not need to improve humans' created content directly. 
They only need to point out the problems or provide suggestions based on understanding humans' created content.
Then humans can decide how to fix the problem or which suggestion is adopted.

The fourth role of AI collaborators is the \textbf{assistant}.
Compared to the previous roles, AI collaborators take even less work when acting as assistants.
They are not authorized to modify anything created by humans and do not need to understand the content.
\revise{Instead, they provide assistance, such as recommending potential actions or answering users' questions, on specific sub-tasks according to humans' requirements or instructions.
The difference between assistants' recommendations and reviewers' suggestions is that reviewers provide suggestions based on the understanding of human-created content while assistants recommend potential actions based on humans' instructions.
Therefore, assistants do not need to understand human-created content.}

% \haotian{I updated this part.}



% provide assistance on specific tasks according to humans' requirements.
% \haotian{How do we make it clearer? A reviewer mentioned that the final sentence is too general that can also be used for other roles.}


We further assess the four roles using the \textit{``agency vs. automation''} framework~\cite{heer2019agency}.
The framework is derived from the ideal goal of human-AI collaborative tools, achieving \textit{``agency plus automation''}, 
\re{The framework is derived from the ideal goal of human-AI collaborative tools, achieving \textit{``agency plus automation''}, where both the automation brought by AI usage (\ie, \textit{automation}) and the control of humans (\ie, \textit{agency}) could be maximized as much as possible.
In this way, humans can spend minimum effort on tasks while maintaining a high level of control to achieve their target.}
% where AI automates the tasks (\ie, \textit{automation}) under humans' control (\ie, \textit{agency}).
According to Heer~\cite{heer2019agency}, tool designers may need to estimate human-AI collaborative tools' levels of agency and automation and examine if they fit users' tasks and requirements.
Following this idea, we characterize the four roles of AI summarized from the interview using the agency and automation levels when humans collaborate with different AI collaborators.
Fig.~\ref{fig:task-role}(a) shows the estimated levels of human agency and AI automation of four AI roles and two anchor points, \ie, fully manual data storytelling without AI and the ideal ``agency plus automation''. 

When AI collaborators serve as creators, humans have little control over how AI performs tasks and AI fully automates the task.
Therefore, it has the lowest level of agency among the four roles, while the level of automation is the highest.
We consider that its level of automation is close to ``agency plus automation'' while its level of agency is close to zero.
When working with AI optimizers, humans have a higher agency but take more workload.
AI optimizers only automate content improvement based on understanding humans' input.
AI assistants have a lower level of automation since it only reacts to specific requirements given by humans.
We consider that when AI collaborators serve as reviewers, both their level of automation and human collaborators' level of agency are between those of assistants and creators because AI reviewers need to understand the input by themselves and may not execute an optimization plan automatically.
Moreover, reviewers do not directly follow humans' instructions but give humans control over whether and how they follow the advice. 
\revise{To summarize, we consider that the role of creators allows AI to take more automated actions while being less controlled by humans.
Therefore, it is the role in the area where AI automation weighs more than human agency.
On the other hand, when collaborating with AI systems as assistants, reviewers, and optimizers, humans take control of the collaboration and therefore these roles are in the area where human agency is emphasized over automation.}


\begin{table*}[]
\centering
\footnotesize
\caption{This table provides \re{definitions and examples of AI's expected behavior under different roles} in all tasks of the data storytelling workflow. Some combinations (indicated with italic fonts) of AI's roles and tasks were not proposed by our interviewees, which does not indicate that those combinations are not possible. Sec.~\ref{sec:discussion_limitation} discusses the potential AI behaviors in these combinations.}
\begin{tabular}{@{}p{3.2cm}p{3.2cm}p{3.2cm}p{3.2cm}p{3.2cm}@{}}
\toprule
 \textbf{Task}                         & \textbf{Creator}: the AI collaborator who finishes the task independently                                                                                                       & \textbf{Optimizer}: the AI collaborator who improves manually created content                                                       & \textbf{Assistant}: the AI collaborator who assists creation according to humans' requests                                                                                                                                             & \textbf{Reviewer}: the AI collaborator who evaluates manually created content and provides suggestions                                                                                                      \\ \midrule
Decide the core message   & Automatically decide the core message                                                                         & \textit{No participant mentions AI’s expected behavior under the role in the task}                                                & Summarize the goal from the analysis results, provide some potential ideas for inspiration                                                                & Summarize the resulting data story and check if the message in the summarization aligns with the author’s original idea \\\midrule
Collect data facts        & Automatically mine data facts from the dataset without instruction from humans                                  & \textit{No participant mentions AI’s expected behavior under the role in the task}                                                & Answer humans' questions about data or suggest data queries
& \textit{No participant mentions AI’s expected behavior under the role in the task}                                                                                                \\\midrule
Compile the story outline & Create an outline according to the current progress of the project                              & Improve the outline from the storytelling technique perspective & Recommend multiple outlines of telling the story for humans’ decisions                                                                                    & Check the logic flow of the outline                                                                           \\\midrule
Prepare story pieces      & Automatically plot charts or add text explanations                                                            & Polish the text or charts.                                      & Auto-complete code, support voice-based input                                                                 & Provide suggestions to improve the clarity, identify factual mistakes.                                      \\\midrule
Integrate story pieces    & Automatically generate the slides                                                                             & \textit{No participant mentions AI’s expected behavior under the role in the task}                                               & Manage the link between charts in slides and data                                                                                                         & \textit{No participant mentions AI’s expected behavior under the role in the task}                                                                                               \\\midrule
Style the data story    & Generate animated transitions, create decorative figures & Beautify the charts and tables        & Suggest layout, manage color usage                                                                                                                        & Evaluate the overall aesthetics and provide scores                                                            \\\midrule
Share the data story      & Create presentation videos                                                                                    & \textit{No participant mentions AI’s expected behavior under the role in the task}                                             & Upload the data story to a cloud server, distribute the data story through email                                                                              & \textit{No participant mentions AI’s expected behavior under the role in the task}                                                                                          \\ \bottomrule
\end{tabular}
\label{tab:roles_tasks}
\end{table*}

==> sources/outdated/07-suggestion-v2.tex <==
\section{What should future human-AI collaborative tools look like?}\label{sec:suggestion}
Our interviewees showed their passion for introducing AI to their workflow.
As discussed in Sec.~\ref{sec:ai_tasks}, they commonly preferred collaborating with AI rather than asking AI to create a story from data in an end-to-end manner.
Based on the observation, we consider that more human-AI collaborative tools should be studied and offered to data workers.
In this section, we propose recommendations for future data storytelling tools according to our findings in the interview. 


\subsection{Adaptive to different contexts and preferences}
We envision that AI in future storytelling tools should consider user-specified contexts and preferences.

Most of the existing AI-powered storytelling tools (\eg, \cite{wang2019datashot, shi2020calliope}) 
only consider the data relationship between story pieces.
However, as indicated in Sec.~\ref{sec:why_not_context}, the lack of considering contexts may hinder their acceptance.
Examples of contexts include the goal of a project, the social background, the authors' previous data stories, and the team members' preferences.
Modeling these contexts can help AI to understand what a data story targets and how the story can be compelling.
As P7 and P16 suggested (see Sec.~\ref{sec:why_feelings}), AI collaborators are ultimately expected to serve as personal assistants so they can learn the contexts of data stories implicitly through their daily actions, which was also mentioned by Horvitz~\cite{horvitz1999principles}.
Another potential approach is to allow users to set up contexts and their preferences explicitly.
For example, P7 imagined that he could use the context of his presentation as part of the input parameters.
He could tell AI his need to
tell a data story formally or informally in different countries.
AI could adjust the story according to the occasion and the audience's cultural background.

Furthermore, as our summary in Fig.~\ref{fig:task-role}(c) indicates, users may prefer different patterns of collaboration, which may be related to their work nature.
For example, the interviewees with business backgrounds considered human-human communication irreplaceable and did not prefer collaborating with AI in the communication stage~(see Sec.~\ref{sec:why_not_human_communication}).
Therefore, the tools should not assume that AI collaborators' roles are fixed and provide the same help to different users.
They can be adaptive to different requirements according to users' configuration.


\subsection{Effective and natural to communicate and interact with}
Our second recommendation is to build effective communication channels between humans and AI by leveraging natural interactions.

Despite mouses and keyboards, more interaction approaches have been explored recently.
For example, SketchStory~\cite{lee2013sketchstory} reveals that sketching can make data stories more engaging.
VisTalk~\cite{wang2022towards} and Falx~\cite{wang2021falx} propose natural language-based and example-based chart authoring.
These tools have the potential to enrich the communication channels in human-AI collaborative data storytelling.

Beyond these tools that support a new modality of communication, we argue that it is promising to enhance communication by combining multiple modalities (see Sec.~\ref{sec:why_not_communicate}).
The idea is inspired by a sequence of research in multi-modal interaction with visualizations~\cite{srinivasan2020interweaving, kim2021data, walny2012understanding}.
For example, 
Srinivasan~\etal~\cite{srinivasan2020interweaving} verified the value of multi-modal interactions in data exploration.
The multi-modal interactions can make the experience closer to human-human communication and better fit the multi-modal nature of data stories~\cite{cheng2022investigating}.
For example, 
users can sketch to indicate their preferred layouts and transitions, while they can indicate their expected emotions in the data story with facial expressions or gestures.
Similarly, AI can present drafts to humans and ask related questions.
Recently, GPT-4~\cite{openai2023gpt4} has taken a step toward multi-modal interaction between humans and AI models.
It allows both images and texts as the input but limits the output to texts only.
When communication is more natural and convenient, concerns about miscommunication and the learning cost of effective communication (see Sec.~\ref{sec:why_not_overhead}) should also be mitigated.

\subsection{Transparent and controllable AI to facilitate users' understanding and steering}
The third design suggestion is to make AI more transparent to users.
Our participants had concerns regarding the black-box nature of AI models, including the unclear and potentially unreliable data sources~(see Sec.~\ref{sec:why_not_data}), the miscommunication between humans and AI collaborators, and consequent responsibility problems (see Sec.~\ref{sec:why_not_ethical}).

A potential way of addressing these concerns is to enhance the explainability of AI~\cite{ehsan2021expanding}.
We imagine that future AI collaborators in data storytelling should be able to explain their actions as human collaborators do.
For example, AI may explain how a generated storyline aligns with design guidelines~(\eg, \cite{bach2018narrative}).
In this way, users can better understand and judge whether AI's actions are reasonable.
We hope that future research could work on explaining AI's behavior in storytelling tools, including what and how to explain.
Furthermore, humans should be provided with functions to steer AI models according to various needs.
For example, to handle the potential data reliability issues, despite providing the source of created content, AI should remove all content without authoritative information sources per users' request.

Another benefit of being transparent is to possibly enhance humans' understanding of their produced data stories~(see Sec.~\ref{sec:workflow}).
For example, if humans and AI have divergent ideas about the data story, AI's explanations may help humans reflect on their understanding and improve their stories.
At the same time, humans' feedback to AI may also help AI understand humans and their context better~\cite{kamar2016directions}.


\subsection{Convenient to adopt and learn for novices}
The last recommendation is that AI-powered tools should be convenient for novice users.
They should have low adoption and learning cost.

As mentioned in Sec.~\ref{sec:why_not_overhead}, configuring AI models can result in overhead that hinders users from using them.
Therefore, we consider it necessary to ease the adoption of tools.
For example, the tools can be web-based applications, similar to ChatGPT, to eliminate the need to deploy AI models locally.
Another potential is to be seamlessly integrated into users' familiar tools, such as PowerPoint plug-ins.
In these ways, novice users can approach helpful AI-powered tools without configuring them from  setting up environments.

The second perspective is to lower the learning cost by having clear instructions when collaborating with AI in these tools.
Recent large AI models (\eg, ChatGPT) can handle various downstream tasks.
However, their boundaries of capabilities, such as the possible tasks and the performances, are unclear.
When dealing with such unclear boundaries, humans may have to figure out if their tasks are feasible for AI with trial and error.
This process can introduce additional overhead
~(see Sec.~\ref{sec:why_not_overhead}).
Furthermore, communicating tasks effectively can be challenging ~(see Sec.~\ref{sec:why_not_communicate}).
To address these issues, we suggest that the developers should prepare clear instructions when designing future human-AI collaborative data storytelling tools.
The instruction should include an estimated boundary of the tools (\ie, tasks and performances) and clear guidelines for the communication approaches.
With instructions, users can be clearer about what and how they can collaborate with AI in these tools.


